A full-resolution training framework for Sentinel-2 image fusion

This work presents a new unsupervised framework for training deep learning models for super-resolution of Sentinel-2 images by fusion of its 10-m and 20-m bands. The proposed scheme avoids the resolution downgrade process needed to generate training data in the supervised case. On the other hand, a proper loss that accounts for cycle-consistency between the network prediction and the input components to be fused is proposed. Despite its unsupervised nature, in our preliminary experiments the proposed scheme has shown promising results in comparison to the supervised approach. Besides, by construction of the proposed loss, the resulting trained network can be ascribed to the class of multi-resolution analysis methods.

==> drawing/preambol.tex <==
\usepackage{tikz,amsmath,amssymb,bm,color}
\usetikzlibrary{shapes,arrows,arrows.meta}
% needed for BB
\usetikzlibrary{patterns}
\usetikzlibrary{fit}
\usetikzlibrary{calc,3d}

\pgfdeclareimage[width=1.6cm]{x10}{./matlab/X10.png}
\pgfdeclareimage[width=8mm]{x20}{./matlab/X20.png}
\pgfdeclareimage[width=8mm]{x10d}{./matlab/X10.png}
\pgfdeclareimage[width=4mm]{x20d}{./matlab/X20.png}
%\pgfdeclareimage[width=1.6cm]{x20u}{./matlab/X20.png}
\pgfdeclareimage[width=1.6cm]{x20u}{./matlab/pred.png}


\tikzstyle{FRAME}=[rectangle,draw,ultra thick, minimum width=1.6cm, minimum height=1.6cm,inner sep=0pt]
\tikzstyle{Frame}=[rectangle,draw, ultra thick,minimum width=0.8cm, minimum height=0.8cm,inner sep=0pt]
\tikzstyle{frame}=[rectangle,draw,very thick, minimum width=0.4cm, minimum height=0.4cm,inner sep=0pt]

\definecolor{col10}{rgb}{0,0.5,0.8}%{0.2, 0.5, 1}
\definecolor{col20}{rgb}{0.8,0.2,0.0}%{0.2, 0.5, 1}%{1, 0.2, 0.2}
\definecolor{colLoss}{rgb}{0.8,0.8,0.2}%{0.2, 0.5, 1}%{1, 0.2, 0.2}

\tikzstyle{BOX}=[rectangle,dashed, draw,minimum width=2.1cm, minimum height=0.8cm,inner sep=0pt]
\tikzstyle{LPF}=[rectangle, draw,minimum width=0.8cm, minimum height=0.4cm,inner sep=0pt]
\tikzstyle{DWN}=[rectangle, draw,minimum width=0.4cm, minimum height=0.4cm,inner sep=0pt]
\tikzstyle{CNN}=[rectangle,draw, very thick, minimum width=1.2cm, minimum height=0.6cm,inner sep=0pt]
\tikzstyle{DET}=[rectangle,draw, thick, minimum width=1.2cm, minimum height=0.6cm,inner sep=1pt]


\tikzstyle{Loss}=[circle, fill=colLoss, very thick,draw, minimum size=0.8cm, inner sep=0pt]
\tikzstyle{SUM}=[circle, thick,draw, minimum size=0.3cm, inner sep=0pt]
\tikzstyle{arr}=[thick, -stealth]

